A projection-based, semi-implicit time-stepping approach for the Cahn-Hilliard Navier-Stokes equations on adaptive octree meshes

The Cahn-Hilliard Navier-Stokes (CHNS) system provides a computationally tractable model that can be used to effectively capture interfacial dynamics in two-phase fluid flows. In this work, we present a semi-implicit, projection-based finite element framework for solving the CHNS system. We use a projection-based semi-implicit time discretization for the Navier-Stokes equation and a fully-implicit time discretization for the Cahn-Hilliard equation. We use a conforming continuous Galerkin (cG) finite element method in space equipped with a residual-based variational multiscale (RBVMS) formulation. Pressure is decoupled using a projection step, which results in two linear positive semi-definite systems for velocity and pressure, instead of the saddle point system of a pressure-stabilized method. All the linear systems are solved using an efficient and scalable algebraic multigrid (AMG) method. We deploy this approach on a massively parallel numerical implementation using parallel octree-based adaptive meshes. The overall approach allows the use of relatively large time steps with much faster time-to-solve than similar fully-implicit methods. We present comprehensive numerical experiments showing detailed comparisons with results from the literature for canonical cases, including the single bubble rise and Rayleigh-Taylor instability.

==> Scaling.tex <==
% % !TEX root = main.tex
\section{Scaling of the numerical implementation}
\label{sec:scaling}
\subsection{Strong scaling}

We perform a detailed timing analysis to demonstrate the parallel scalability of the framework.  We perform all scaling tests on TACC's~\Stampede~ Knights Landing processors ranging from~1 node to~256 nodes with~68 processors per node.  We study in detail the lid-driven cavity case in~\cref{subsec:ldc_3d} for the scaling analysis.  We run each scaling experiment for ten time steps such that the initialization and setup do not dominate the timing. Three different levels of refinement characterize each mesh: 1. background mesh refinement ($L_{\mathrm{bkg}}$); 2. wall refinement ($L_{\mathrm{wall}}$); and 3. interface refinement ($L_{\mathrm{interface}}$). As the interface evolves, the mesh is subsequently refined near the interface and coarsened away from it.  \Cref{tab:refinement} shows the level of refinement and the approximate number of total elements for each of the three different meshes used for the scaling study.
%
\begin{table}[H]
\centering
\normalsize
\resizebox{0.3\linewidth}{!}{%
\begin{tabular}{|c|ccc|c|}
\hline
\hline
& $L_{\mathrm{bkg}}$ & $L_{\mathrm{wall}}$ & $L_{\mathrm{interface}}$ & $N_{\mathrm{elem}}$ \\ \hline
\textsc{M1} & 3 & 5 & 7 & 280 K\\
\textsc{M2} & 4 & 6 & 8 & 1 M\\
\textsc{M3} & 5 & 7 & 9 & 19 M\\
\hline
\end{tabular}%
}
\caption{Level of refinements involved in different meshes used for scaling studies}
\label{tab:refinement}
\end{table}

Panel~(a) of~\cref{fig:strong_scaling} shows the result of strong scaling for three different meshes, and panel~(b) shows the corresponding relative speedup. \Cref{fig:strong_scaling} demonstrates that we achieve a better than ideal scaling for these cases. To analyze the reasons behind this, we analyze component-by-component the framework timings and observe that the two dominant ones in the total run time are the Jacobian assembly ($J$ in~\cref{sec:numerical_tecniques}) and the preconditioner setup (PC setup in~\petsc), with PC setup dominating the timing (see~\cref{fig:scaling-fraction}).  Therefore, to understand the scaling behavior, we plot the strong scaling curves and corresponding relative speed up for these two components in~\cref{fig: strongScalingDetailed}.   Panels~(a) and~(b) of~\cref{fig: strongScalingDetailed} detail the scaling for Jacobian assembly, whereas, panels~(c) and~(d) show the scaling for PC setup.  As expected, the Jacobian assembly scales almost ideally for all the cases considered from panels~(a) and~(b) of~\cref{fig: strongScalingDetailed}.  However, the PC setup has better than ideal scaling, see panels~(c) and~(d).  As the PC setup dominates the total solution time, the overall scaling mimics this behavior.  

\input{Figures/ScalingTikz/StrongScaling}
The deep memory hierarchy inherent in modern-day clusters may be the cause for the better than ideal scaling behavior.  We use an additive Schwarz-based block preconditioning with each block using LU  factorization (-\texttt{sub\_pc\_type} in~\petsc) (see~\ref{sec:app_linear_solve}) to compute the factors of the block matrix. The factorized block preconditioned matrix loses its sparsity, and the resultant matrix is less sparse ($b \times b$) matrix, where $b$ is the block size of the matrix on a processor. This denser matrix can no longer fit in L1, L2, or L3 cache for a big enough problem size. As the number of processors increases, the resulting problem size in a processor diminishes. Thus, these denser blocks begin to fit in cache, and therefore, we achieve a better than ideal speedup for PC setup and subsequent solve time. 

Figure~\ref{fig:scaling-fraction} shows the relative fraction of time spent in different meshes. 
%We see that PC setup is the most time-consuming step. 
%
We observe two specific trends. First, as the number of processors increases such that number of elements remains constant, the relative cost of PC setup decreases. This is because of the fact that LU factorization is performed on a smaller block matrix. Also, the cost of communication while performing matrix assembly and vector assembly increases with increase in number of processor, whereas LU factorization is performed on a block matrix and thus requires no communication. Secondly, increasing the number of elements such that the number of processor is fixed has a substantial effect on the relative cost of PC setup. LU factorization is an $\mathcal{O}(N^3)$ operation, whereas the number of FLOPS and communication involved in other operations like matrix assembly is atmost $\mathcal{O}(N^2)$. This explains the increase in the PC setup cost.
%
Future work will seek to develop schemes that will efficiently use cheaper preconditioners, whilst maintaining the energy stability and mass conservation of these schemes.

\input{Figures/ScalingTikz/Components}
\begin{remark}
We use a Krylov space solver (BCGS) with ASM/LU preconditioning. Therefore, algebraic multi-grid solvers with \petsc's AMG can substantially improve the solve time.  Although we had some success with this setup (e.g., the 2D Rayleigh Taylor in~\cref{subsec:rayleigh_taylor_2D} cases use this setup), the 3D examples use the ASM/LU combination.  %And, as they are very expensive large scale cases and very expensive to re-run, we chose to show scaling analysis for the ASM/LU combination.  
\end{remark}
 
\subsection{Weak scaling}
Performing exact weak scaling \footnote{Weak scaling studies the variation in simulation time as we increase the number of processors with a fixed problem size per processor.} is non--trivial due to the adaptive nature of the mesh. Therefore, we consider  simulations with an approximately equal number of elements per processor to deduce the weak scaling nature of our solver.  \Cref{fig:weakScaling} shows the weak scaling results for the different problem sizes. Overall, similar to the strong scaling, we see an excellent weak scaling efficiency for different problem sizes. For each of the cases, we observe a weak scaling efficiency of greater than 0.5 for a 64 fold increase in the problem size. We also analyze the weak scaling for the dominant components of the overall time, i.e. Jacobian assembly and PC setup.  \Cref{fig:weakScalingDetailed} segregates the time for these components. The weak scaling efficiency ($> 0.5$) for each of these individual components is excellent as we vary the problem size by two orders of magnitude.
\input{Figures/ScalingTikz/WeakScaling}
The preconditioner complexity and cost challenges (as seen from~\cref{fig:scaling-fraction}) are also present in the block iterative method of~\citet{ Khanwale2020},  where one performs these operation multiple times within one timestep (once every block iteration). This combined cost makes the block iterative method much more expensive compared to the fully coupled solver. Therefore, the current coupled framework improves the overall time to solve by reducing the number of evaluations required for Jacobian assembly and PC setup. In challenging application problems, preconditioning the linear problem (sub-iteration within each Newton solve)  requires substantial computational effort; future work will seek improve the speed and efficiencies of the preconditioning.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Deleted part 
% %\begin{figure}[H]
% %\begin{tikzpicture}
% %	\centering
% %  \begin{groupplot}[
% %      group style={group size=3 by 1,ylabels at=edge left,vertical sep=10pt},
% %      ylabel style={text height=0.02\textwidth,inner ysep=0pt},
% %      xlabel= Number of processors, % Set the labels
% %      ylabel= Time (in s),
% %      xtick={256,1000,4000,17000},
% %      xticklabels={$256$,$1K$,$4K$,$17K$},
% %      height=0.35*\linewidth,width=0.35\linewidth,/tikz/font=\small,
% %    %   xtick={512,2000,8000,32000},
% %    %   xticklabels={$512$,$2K$,$8K$,$32K$},
% %    ]
% %     \nextgroupplot[xmode=log,log basis x={2},ymode=log,title={\textbf{Jacobian}},ytick={20,80,320},yticklabels={$20$,$80$,$320$}]%
% %     \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={\thisrow{Jacobian}},col sep=space]{Figures/ScalingData/3LvlNew.txt};
% %        \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={\thisrow{Jacobian}},col sep=space]{Figures/ScalingData/4Lvl.txt};
% %         \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={\thisrow{Jacobian}},col sep=space]{Figures/ScalingData/5Lvl.txt};
% %         \coordinate (top) at (rel axis cs:0,1);% coordinate at top of the first plot
% %    
% %    %  \nextgroupplot[xmode=log,log basis x={2},ymode=log,title={\textbf{Residual}}]%
% %    %  \addplot
% %    %      table[x expr={\thisrow{Proc}))},y expr={\thisrow{VecAssembly}},col sep=space]{Figures/ScalingData/3Lvl.txt};
% %    %     \addplot
% %    %      table[x expr={\thisrow{Proc}))},y expr={\thisrow{VecAssembly}},col sep=space]{Figures/ScalingData/4Lvl.txt};
% %    %      \addplot
% %    %      table[x expr={\thisrow{Proc}))},y expr={\thisrow{VecAssembly}},col sep=space]{Figures/ScalingData/5Lvl.txt};
% %    % \coordinate (bot) at (rel axis cs:1,0);% coordinate at bottom of the last plot
% %    
% %     \nextgroupplot[xmode=log,log basis x={2},ymode=log,title={\textbf{PC Setup}}]%
% %     \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={\thisrow{PCSetUp}},col sep=space]{Figures/ScalingData/3LvlNew.txt};
% %        \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={\thisrow{PCSetUp}},col sep=space]{Figures/ScalingData/4Lvl.txt};
% %         \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={\thisrow{PCSetUp}},col sep=space]{Figures/ScalingData/5Lvl.txt};
% %     
% %    
% %    \nextgroupplot[xmode=log,log basis x={2},ymode=log,title={\textbf{Total time}}]%
% %     \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={\thisrow{Solve}},col sep=space]{Figures/ScalingData/3LvlNew.txt};\label{plot:leveldet3}
% %        \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={\thisrow{Solve}},col sep=space]{Figures/ScalingData/4Lvl.txt};\label{plot:leveldet4}
% %         \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={\thisrow{Solve}},col sep=space]{Figures/ScalingData/5Lvl.txt};\label{plot:leveldet5}
% %    \coordinate (bot) at (rel axis cs:1,0);% coordinate at bottom of the last plot
% %    \end{groupplot}
% %     \path (top|-current bounding box.south)--
% %        coordinate(legendpos)
% %        (bot|-current bounding box.south);
% %  \matrix[
% %      matrix of nodes,
% %      anchor=north,
% %      draw,
% %      inner sep=0.2em,
% %    ]at([yshift=-1ex]legendpos)
% %    { \ref{plot:leveldet3}& \textsc{M1} &[5pt]
% %      \ref{plot:leveldet4}& \textsc{M2} &[5pt]
% %      \ref{plot:leveldet5}& \textsc{M3} &[5pt]\\};
% %\end{tikzpicture}
% %\caption{\textit{Strong scaling:} Figure showing the segregated strong scaling behaviour of two major component of our solver on \Stampede~ Knights Landing processor: Jacobian Assembly and  Preconditioner setup, along with the total solve time. Three different mesh are considered: \textsc{M1} with 280 K elements, \textsc{M2} with 1 M elements and \textsc{M3} with 19 M elements. Excellent scaling behaviour is observed till $\mathcal{O}(17K)$ processor.}
% %\end{figure}

% %\begin{figure}[H]
% %\begin{tikzpicture}
% %	\centering
% %  \begin{groupplot}[
% %      group style={group size=3 by 1,ylabels at=edge left,vertical sep=10pt},
% %      ylabel style={text height=0.02\textwidth,inner ysep=0pt},
% %      xlabel= Number of processors, % Set the labels
% %      ylabel= Time (in s),
% %      xtick={256,1000,4000,17000},
% %      xticklabels={$256$,$1K$,$4K$,$17K$},
% %      height=0.35*\linewidth,width=0.35\linewidth,/tikz/font=\small,
% %    %   xtick={512,2000,8000,32000},
% %    %   xticklabels={$512$,$2K$,$8K$,$32K$},
% %    ]
% %     \nextgroupplot[xmode=log,log basis x={2},ymode=log,title={\textbf{Jacobian}}]%
% %     \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={1.01E+02/\thisrow{Jacobian}},col sep=space]{Figures/ScalingData/3LvlNew.txt};
% %        \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={2.62E+02*4/\thisrow{Jacobian}},col sep=space]{Figures/ScalingData/4Lvl.txt};
% %         \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={1.61E+02*32/\thisrow{Jacobian}},col sep=space]{Figures/ScalingData/5Lvl.txt};
% %    \addplot [no markers, color=black, thick,dashed ] table {
% %        136 1
% %        17408 128
% %        };
% %    \coordinate (top) at (rel axis cs:0,1);% coordinate at top of the first plot
% %    
% %     \nextgroupplot[xmode=log,log basis x={2},ymode=log,title={\textbf{PC Setup}}]%
% %     \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={7.61E+02/\thisrow{PCSetUp}},col sep=space]{Figures/ScalingData/3LvlNew.txt};
% %        \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={4.00E+03*4/\thisrow{PCSetUp}},col sep=space]{Figures/ScalingData/4Lvl.txt};
% %         \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={1.92E+03*32/\thisrow{PCSetUp}},col sep=space]{Figures/ScalingData/5Lvl.txt};
% %    \addplot [no markers, color=black, thick,dashed ] table {
% %        136 1
% %        17408 128
% %        };
% %     
% %    
% %    \nextgroupplot[xmode=log,log basis x={2},ymode=log,title={\textbf{Total time}}]%
% %     \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={9.80E+02/\thisrow{Solve}},col sep=space]{Figures/ScalingData/3LvlNew.txt};\label{plot:Rellevel3}
% %        \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={4.60E+03*4/\thisrow{Solve}},col sep=space]{Figures/ScalingData/4Lvl.txt};\label{plot:Rellevel4}
% %         \addplot
% %         table[x expr={\thisrow{Proc}))},y expr={2.66E+03*32/\thisrow{Solve}},col sep=space]{Figures/ScalingData/5Lvl.txt};\label{plot:Rellevel5}
% %    \addplot [no markers, color=black, thick,dashed ] table {
% %        136 1
% %        17408 128
% %        };\label{plot:Relideal}
% %    \coordinate (bot) at (rel axis cs:1,0);% coordinate at bottom of the last plot
% %    \end{groupplot}
% %     \path (top|-current bounding box.south)--
% %        coordinate(legendpos)
% %        (bot|-current bounding box.south);
% %  \matrix[
% %      matrix of nodes,
% %      anchor=north,
% %      draw,
% %      inner sep=0.2em,
% %    ]at([yshift=-1ex]legendpos)
% %    { \ref{plot:Rellevel3}& \textsc{M1} &[5pt]
% %      \ref{plot:Rellevel4}& \textsc{M2} &[5pt]
% %      \ref{plot:Rellevel5}& \textsc{M3} &[5pt]
% %      \ref{plot:Relideal}& ideal &[5pt]\\};
% %\end{tikzpicture}
% %\caption{\textit{Relative speedup:} Relative speedup for solve time  as a function of number of processor for different problem size. }\label{fig: RelativeSpeedup}
% %\end{figure}

==> dendro.tex <==
% !TEX root = methods_paper.tex

While the concept of adaptive space partitions is well studied, developing such methods for applications demanding frequent refinements on large distributed systems presents significant challenges. This work builds on existing methods for performing large-scale finite element computations using octree-refined meshes. 
The octree-based framework, \dendro\, is extended to support sub-domains, primarily with the objective of supporting long channels and division of the domain based on arbitrary functions that define the geometry.
We provide a brief description on building the octree mesh in parallel and performing finite element computations. Additional details can be found in~\cite{SundarSampathBiros08}. 
% 
\dendro\ provides the adaptive mesh refinement (AMR) and all parallel data-structures, and for this project, \dendro\ was extended to support domains that are not cuboidal in shape. We give a brief overview of the \dendro\ framework and provide details on the new contributions. The main steps in building and maintaining an adaptively refined mesh in a distributed-memory machine are described below.

\paragraph{Refinement:} The sparse grid is constructed based on the geometry. Proceeding in a top-down fashion, a cell is refined if a surface (defined by a zero level-set of a function, or a cloud of points)  passes through it. 
%
We also provide an additional function that tests for membership and eliminates regions outside the domain. This is necessary as by definition the octree maps to a cuboidal domain. By eliminating regions, we can support arbitrary domains, including domains with holes, such a porous media. 
%
% During the same step, we also determine if the cell is completely inside the pillar, and eliminate it from the mesh in that case.   
Since the refinement happens in an element-local fashion, this step is embarrassingly parallel.
The user passes a function that given coordinates, $x,y,z$ returns the distance from the surface. The eight corners of an octant are tested using this function. If all $8$ points have a positive distance (outside), then we retain this element, but do not refine further. If all $8$ points have a negative distance (inside), then this element is removed from the mesh. If some of the corners of the octant are inside and others outside, then this octant is refined. This is repeated till the desired level of refinement is achieved.  
In distributed memory, all processes start from the root and refine until at least $p$ octants requiring further refinement are produced. Then using a weighted space-filling-curve (SFC) based partitioning, we partition the octants. Note that we do not communicate the octants as every process has a copy of the octants, and all that needs to be done at each process is to retain a subset of the current octants and recurse. Since we use finite element, a 2:1 balancing is enforced following the refinement operation. 

\paragraph{2:1 Balancing:} We enforce a condition in our distributed octrees that no two neighbouring octants differ in size by more than a factor of two. This makes subsequent operations simpler without affecting the adaptive properties. Our balancing algorithm is similar to existing approaches for balancing octrees \cite{bern1999parallel,BursteddeWilcoxGhattas11,SundarSampathAdavaniEtAl07} with the added aspect that it does not generate octants if the ancestor does not exist in the input. This is done to ensure that regions that were previously eliminated are not filled in. The algorithm proposed by \citet{bern1999parallel} is easily extensible to support this case, as we simply need to skip adding balancing octants that violate the criteria.

\paragraph{Partition:} Refinement and the subsequent 2:1 balancing of the octree can result in a non-uniform distribution of elements across the processes, leading to load imbalance. This is particularly challenging when arbitrary geometries are meshed, as this can make the mesh heavily load-imbalanced.  The Morton ordering enables us to equipartition the elements by performing a parallel scan on the number of elements on each process followed by point-to-point communication to redistribute the elements.  As we refine near the two-phase interface, it can affect the performance, as it is likely localized on a small subset of processes, this where Morton ordering comes to rescue and delivers and effective partition. The partitioning scheme is able to handle arbitrary geometries as the partition only tries to equally divide the retained elements across the processes.  The weighted partitioning, is a straightforward extension of our SFC-based partitioning that provides variable weight to the elements based on whether the element lies inside the retained domain of the arbitrary geometry or not. This allows us to more accurately estimate the work on each partition and provide better parallel load-balancing.
 

\paragraph{Meshing:} By meshing we refer to the construction of the (numerical) data structures required for finite element computations from the (topological) octree data. \dendro ~already has efficient implementations for building the required neighbourhood information and for managing overlapping domains between processors (\textit{ghost} or \textit{halo} regions). The key difference with our previous applications is the requirement to handle arbitrary geometries, as all neighbours might not be present in the mesh. This also complicates the process of applying boundary conditions. We added support for defining {\em subdomains} within \dendro. The subdomains are defined using a function that takes a coordinate $(x,y,z)$ as input and returns \texttt{true} or \texttt{false} depending on whether that coordinate is part of the subdomain or not. The subdomain leverages the core mesh data-structure and additionally defines a unique mapping for nodes that are part of the subdomain. It also keeps track of which nodes belong to subdomain boundaries. Therefore, subdomains have a small overhead and store significantly less data than the main mesh data-structure. For our target application, it is important to identify the external (domain) boundary as this dictates which elements will be retained in the domain. Therefore, the subdomain stores two \texttt{bits} to keep track of whether a node is non-boundary, or external. 

\paragraph{Handling hanging nodes:} While the use of quasi-structured grids such as octree-grids makes parallel meshing scalable and efficient, without sacrificing adaptivity, one challenge is to efficiently handle the resulting non-conformity. This results in so called {\em hanging nodes} occurring on faces/edges shared between unequal elements that do not represent independent degrees of freedom. In order to minimize the memory footprint and overall efficiency, the hanging nodes are not stored in \dendro. Instead, since they are constrained by the order of the elements and the non-hanging nodes on the hanging face/edge, we introduce these as temporary variable before elemental matrix assembly or matrix-vector multiplication\footnote{for Matrix-free computations} and eliminate them following the elemental operation. This is fairly straightforward given that our meshes are limited to a 2:1 balance, limiting the number of overall cases to be considered. Additional details on the handling of hanging nodes in \dendro\ can be found in \cite{SundarSampathAdavaniEtAl07}. 

\paragraph{Intergrid transfers}

An essential requirement is to adapt the spatial mesh as the interface moves across the domain. An example of the adaptive mesh refinement following the moving bubble is shown in Figure~\ref{fig:mesh_adaption}. In the distributed memory setting, this also indicates a need to repartition and rebalance the load. Every few time steps, we remesh. This is similar to the initial mesh generation and refinement, except that it is now based on the current position of the interface as well as the original geometry. 
%
This is followed by the 2:1 balance enforcement and meshing. Once the new mesh is generated, we transfer the velocity field from the old mesh to the new mesh using interpolation as needed. Since the intergrid transfer happens only between parent and child (for coarsening and refinement) or remains unchanged, this can be performed on the old mesh using standard polynomial interpolation, followed by a simple repartitioning based on the new mesh (Note that the use of SFCs makes this a linear shift). 
%
% The nodes of the local new mesh are distributed over processes based on the old mesh partitioning to perform interpolation. However again, the intergrid transfer is challenging in unstructured meshes as repartitioning usually offers no guarantee of good overlap between the old and new partitions in most graph-based approaches. The distribution of the nodes of local new mesh would be difficult across complex process boundaries. One way to address it may be to reconstruct the global old mesh in each process, and interpolate for the local new mesh based on the global old mesh, which is memory and time consuming.
